Classification and Disease Localization in Histopathology Using Only Global Labels: A Weakly-Supervised Approach

Analysis of histopathology slides is a critical step for many diagnoses, and in particular in oncology where it defines the gold standard. In the case of digital histopathological analysis, highly trained pathologists must review vast whole-slide-images of extreme digital resolution ($100,000^2$ pixels) across multiple zoom levels in order to locate abnormal regions of cells, or in some cases single cells, out of millions. The application of deep learning to this problem is hampered not only by small sample sizes, as typical datasets contain only a few hundred samples, but also by the generation of ground-truth localized annotations for training interpretable classification and segmentation models. We propose a method for disease localization in the context of weakly supervised learning, where only image-level labels are available during training. Even without pixel-level annotations, we are able to demonstrate performance comparable with models trained with strong annotations on the Camelyon-16 lymph node metastases detection challenge. We accomplish this through the use of pre-trained deep convolutional networks, feature embedding, as well as learning via top instances and negative evidence, a multiple instance learning technique from the field of semantic segmentation and object detection.

==> Makefile <==
FILENAME = main
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf
LOG_FILE = $(FILENAME).log

PAPERSIZE = a4

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE) *.tdo *.out *.fls *.synctex.gz *.fdb_latexmk
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	pdflatex -jobname $(FILENAME) main
	find . -regex ".*aux" | while read auxfile; \
	do \
		if grep citation $$auxfile; then \
		echo $$auxfile >> bibbuild.log; \
		echo "------------------------" >> bibbuild.log; \
		bibtex $$auxfile >> bibbuild.log; \
		echo " " >> bibbuild.log;\
		fi; \
	done
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log	
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log

arxiv: main
	cp 
	rm *.toc
	rm *.pdf
	rm *.log
	rm *.blg
	rm *.aux


dvi2pdf:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.4 \
		$(PS_FILE) $(PDF_FILE)

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

print: main
	dvips main

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

compress: clean
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Compressing files in $$i" ; \
	for j in $(COMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(COMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

uncompress:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo Uncompressing files in $$i ; \
	for j in $(UNCOMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(UNCOMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

